Floquet-induced interactions in many-body systems

The development of future quantum devices requires understanding the dynamics of driven many-body systems, in which the Floquet-induced interactions play a central role. This understanding is crucial for coherently controlling quantum states, minimising errors, and benchmarking the performance of these devices. In this thesis, we analyse the enhancement on the Floquet-induced interactions by many-body correlations, and develop an advanced Floquet method to understand the Floquet-induced interactions relevant for future quantum devices.

==> Chapters/abandoned_tex.tex <==
\newenvironment{dedication}
{
    \cleardoublepage
    \thispagestyle{empty}
    \vspace*{\stretch{2}}
    \hfill \begin{center}\begin{minipage}[t]{0.8\textwidth}
    }
    {
    \end{minipage}\end{center}\vspace*{\stretch{3}}\clearpage
}

\newcommand\blankpage{%
    \null
    \thispagestyle{empty}%
    %\addtocounter{page}{-1}%
    \newpage}






\section{Background physics and techniques:}


\subsection{charge-light interaction in Coulomb gauge}

In the Coulomb gauge, there are instantaneous longitudinal interactions between electrons (i.e., the Coulomb interaction); this instantaneous feature is compensated by the coupling between electrons and the vector potential of the environmental electromagnetic modes, which mediates an additional retarded interaction that cures the instantaneous interacting problem, such that the overall interaction between electrons propagates within light cone. This means that the environmental electromagnetic modes, apart from giving rise to the spontaneous decay in the material, also play an important role in preserving the causality of interactions in the material. 



\subsection{commutator as inner derivative}

First, the commutator works like a derivative. Second, the commutator of Fermionic operators can be understood as assembling two sub-branches into a bigger one, with a shared branch contracted. This picture of commutator requires one of the two commuted terms has "cdag-c" balance (i.e., having equal amounts of fermionic creation and annihilation operators). This diagrammatic illustration of commutator calculation is similar to Feynman diagrams. However, in each diagram generated here, there is no internal frequency (i.e. Matsubara frequency) to sum over.

\subsection{Momentum space thermal Feynman diagrams}
The momentum-space thermal Feynman diagram method used in the Matsubara formalism treats the condensed matter system from a high-temperature point of view.

Here, we start from a free electron system and perturbatively add the influence of the interactions. At high temperatures, the kinetic energy of the electrons dominates the interaction energy, and thus, the free electron picture is already close to the accurate description.  This means the perturbation converges quickly at high temperatures. However, as the temperature decreases to some critical values, the interaction begins to dominate, which makes the previous free-electron picture no longer a good starting point from which to perturb. Mathematically, this leads to divergences in Feynman diagram resummation at low temperatures.

In this high-temperature picture (i.e., perturbing from the non-interacting model), we estimate the critical temperature by calculating when the resummation diverges. However, to predict the behaviour below the critical temperature, we usually need to switch to a low-temperature picture where an interacting model becomes the starting point of perturbation. For example, using the momentum-space Feynman diagram method, we can estimate the critical temperature $Tc$ for the pairing instability in a superconductor. However, this high-temperature picture becomes less powerful if we want to know whether these pairs condensed below $Tc$.

Thus, developing many-body analytical methods (e.g., to calculate the electronic behaviours such as the response functions) which go beyond the momentum-space Feynman diagram methods will provide a better understanding of the many-body physics from a low-temperature point of view. The FSWT constructed in the second part of the thesis shows the potential of achieving this development since the Sylvester equation can be solved without being perturbed from a non-interacting model. 





%thw following paragraph should not exist in introduction
\paragraph{The advantage of Floquet approaches compared with the co-rotating frame RWA approach}
%why Floquet theory is better than The rotating wave approximation in co-rotating frames
In the co-rotating frame, adiabatic elimination has been widely used to find the effective Hamiltonian, which describes the laser's dressing effect on the undriven system. In this co-rotating frame, the equilibrium state Feynman diagram method can also be used to obtain the driving-induced phase transitions.
There are two drawbacks to the co-rotating frame approach. First, we ignored the counter-rotating part, which still oscillates in the rotating frame. Finding a rotating frame in which the oscillation is completely cancelled is often challenging. Second, we cannot guarantee the driven system will follow the thermal distribution given by the effective static Hamiltonian in this rotating frame.

Below, we discuss the problem of Adiabatic elimination in a two-band system with chemical potential and show that the Floquet theory works better in this system. 
Eliminating an electron annihilation operator of the upper band gives an effective Hamiltonian, but this Hamiltonian depends on the upper band's detuning to the chemical potential but not on the bandgap between two bands. Floquet theory, on the other hand, doesn't have this issue.  

For the adiabatic elimination paper, cite Alessio's "Cavity-mediated quantum spin liquid" and point out the problem of adiabatic elimination in a strongly correlated system. A similar problem appears in Hongmin's Schrieffer Wolff transform derivation of the cavity-mediated interaction in a Coulomb electron gas. 

Intrinsic interactions must be taken into account when working with driving. Many-body Floquet theory is a compact method that treats every term in the Hamiltonian on equal foot, leading to Floquet-induced interactions.

We will see that in driven Hubbard models, the driving-induced 3-electron interaction plays an essential role in accurately describing the driven dynamics. The Floquet Schrieffer Wolff transform in Chapter 4 generates these driving-induced interactions systematically. On the contrary, to capture this process using Feynman diagrams, we have to sum over 3-particle diagrams to infinite orders, which is tedious.


\section{\textcolor{blue}{Appendix for Pomeranchuk}}\label{appendix-chap5}

We will estimate the criteria for the cavity-mediated Pomeranchuk instability in our driven cavity-QED setup. As an estimation, we only consider the on-site repulsion as in Chapter 3. Besides, we will also treat the cavity-independent Floquet-induced interaction $\hat{H}_{\text{cav-indep FII}}$ at mean-field level, such that the influence of $\hat{H}_{\text{cav-indep FII}}$ is approximated by the excitonic enhancement on the AC Stark shift, as discussed in Chapter 3. Within this mean-field treatment, we estimate that the Pomeranchuk instability can be triggered by the cavity-mediated interaction at a temperature around 1 Kelvin. Near this critical temperature, more rigorous analysis must be conducted in future works, where the cavity-independent Floquet-induced interaction is treated on equal foot with the cavity-mediated interaction.

\subsection{Estimationn of the criteria for the cavity-mediated Pomeranchuk instability}\label{appendix:Pomeranchuk-criteria}
 
Considering only the forward scattering part of the cavity-mediated interaction in the lower-band, the effective Floquet Hamiltonian Eq.~(\ref{eq.main-result}) becomes
\begin{equation}
    \hat{H}^{\text{eff}} = \sum\limits_{{\bf k},s} (\ep_{{\bf k},1}^{d,U}-\mu) \hat{n}_{{\bf k},s} + \sum\limits_{{\bf k},{\bf k'},s,s'} f({\bf k},{\bf k'}) \hat{n}_{{\bf k},s} \hat{n}_{{\bf k'},s'}
\end{equation}
where the Floquet band structure $\ep_{{\bf k},1}^{d,U}$ is defined in Eq.~(\ref{eq.h_eff}), and the cavity-mediated forward interaction $f({\bf k},{\bf k'})$ is defined in Eq.~(\ref{eq.U_eff}). Under 0 temperature, assuming no Fermi surface instabilities appear, in our square lattice, the Landau free-energy of the system reads
\begin{equation}\label{LandauFreeEnergy}
    \Omega = \frac{N}{4\pi^2} \sum\limits_{s} \int_{\bf k} (\ep_{{\bf k},1}^{d,U}-\mu) n_{{\bf k},s}
    ~ + ~  \bigg(\frac{N}{4\pi^2}\bigg)^2 \sum\limits_{s,s'} \int_{\bf k}\int_{\bf k'} f({\bf k},{\bf k'}) n_{{\bf k},s} n_{{\bf k'},s'},
\end{equation}
where $N$ is the total lattice number, $4\pi^2$ is the area of the First Brillioun zone that the integration runs over, and $n_{{\bf k},s} = \langle \hat{c}_{{\bf k} 1 s}^{\dag}  \hat{c}_{{\bf k} 1 s} \rangle$ is the local occupancy in the lower-band at ${(\bf k},s)$. We perturb this local occupancy from the following Fermi distribution by a deviation $\delta n_{{\bf k},s}$, such that
\begin{equation}\label{FermiSurfaceVariance}
    n_{{\bf k},s} = n_F( \ep_{{\bf k},1}^{d,U} - \mu ) + \delta n_{{\bf k},s} 
\end{equation}
where the Fermi function reads $n_F(x) = \frac{1}{1+\exp(\beta x)}$, and the inverse temperature $\beta\to\infty$. 

Here $n_F( \ep_{{\bf k},1}^{d,U} - \mu )$ describes the Fermi surface of the driven material without cavity. Without cavity, this Fermi surface remains to be the same tiny circle ($k_F=\pi/30$) identical to the non-driven case, as long as the driving is not strong enough to create the van Hove singularity (i.e. inverse the band-top). Throughout the calculation, the value of the chemical potential $\mu$ can variate, in order to fix the total electron number in the lower-band. 

After coupling the material to the cavity, as the local occupation is changed from $n_F( \ep_{{\bf k},1}^{d,U}- \mu )$ to Eq.~(\ref{FermiSurfaceVariance}), the free-energy will shift by $\delta \Omega$. This shift can be obtained by inserting Eq.~(\ref{FermiSurfaceVariance}) into Eq.~(\ref{LandauFreeEnergy}), which gives
\begin{equation}\label{deltaOmega}
\begin{split}
    \frac{4\pi^2}{N} \delta \Omega 
    &= \sum\limits_{s} \int_{\bf k} \bigg(\ep_{{\bf k},1}^{d,U} -\mu + \frac{N}{4\pi^2}\sum\limits_{s'} \int_{\bf k'} 2 f({\bf k},{\bf k'})  n_F( \ep_{{\bf k'},1}^{d,U}- \mu )  \bigg) \delta n_{{\bf k},s}
    ~ + ~  \frac{N}{4\pi^2} \sum\limits_{s,s'} \int_{\bf k}\int_{\bf k'} f({\bf k},{\bf k'}) \delta n_{{\bf k},s} \delta n_{{\bf k'},s'} \\
    &\equiv \sum\limits_{s} \int_{\bf k} (\ep^{s}_{\bf k} -\mu) \delta n_{{\bf k},s}
    ~ + ~  \frac{1}{2} \sum\limits_{s,s'} \int_{\bf k}\int_{\bf k'} f^{s,s'}_{{\bf k},{\bf k'}} \delta n_{{\bf k},s} \delta n_{{\bf k'},s'}
\end{split}
\end{equation}
where in the second line we define the Landau interaction function as
\begin{equation}\label{Landau}
    f^{s,s'}_{{\bf k},{\bf k'}} \equiv 2 \frac{N}{4\pi^2} f({\bf k},{\bf k'}) =- \frac{1}{2\pi^2} \frac{\vert g   g_{c,{\bf q}={\bf 0}} \vert^2 }{ \Delta_c} \frac{1}{ \Delta_{{\bf k},s} } \frac{1}{ \Delta_{{\bf k'},s'} },
\end{equation}
and the cavity-shifted single-particle dispersion $\ep^{s}_{\bf k}$ reads
\begin{equation}\label{cavity-shifted-dispersion}
\begin{split}
    \ep^{s}_{\bf k} &\equiv \ep_{{\bf k},1}^{d,U}  + \sum\limits_{s'} \int_{\bf k'} f^{s,s'}_{{\bf k},{\bf k'}}  n_F( \ep_{{\bf k'},1}^{d,U}- \mu ) \\
    &\approx \ep_{{\bf k},1} - \frac{\vert g \vert^2}{\Delta_{{\bf k},s}} 
    - \frac{1}{\pi^2} \frac{\vert g   g_{c,{\bf q}={\bf 0}} \vert^2 }{ \Delta_c} \frac{1}{ \Delta_{{\bf k},s} } \int_{\bf k'} \frac{1}{ \Delta_{{\bf k'},s'} }  n_F( \ep_{{\bf k'},1}^{d,U}- \mu ) \\
    &= \ep_{{\bf k},1} - (1+\eta) \frac{\vert g \vert^2}{\Delta_{{\bf k},s}} \\
    &= (1+\eta) ~ \ep_{{\bf k},1}^{d,U} - \eta ~ \ep_{{\bf k},1}
\end{split}
\end{equation}
where in the second line we use the definition of $\ep_{{\bf k},1}^{d,U}$ in Eq.~(\ref{eq.h_eff}), and omit the contribution from Bloch-Siegert shift. In the third line we define a constant 
\begin{equation}\label{appendix:eta-param}
\eta \equiv \frac{1}{\pi^2} \frac{\vert  g_{c,{\bf q}={\bf 0}} \vert^2 }{ \Delta_c} \int_{\bf k'} \frac{1}{ \Delta_{{\bf k'},s'} }  n_F( \ep_{{\bf k'},1}^{d,U}- \mu ) \\
\approx \frac{1}{\pi^2} \frac{\vert  g_{c,{\bf q}={\bf 0}} \vert^2 }{ \Delta_c} \int_{\bf k'} \frac{1}{ \Delta_{{\bf k'},s'} }.
\end{equation}
Here we can simplify the Fermi distribution to be $n_F=1$, because of the tiny Fermi surface. In the last line of Eq.~(\ref{cavity-shifted-dispersion}) we again use the definition of $\ep_{{\bf k},1}^{d,U}$ and omit the Bloch-Siegert shift. The factor $\eta$ can be understood as an additional self-energy term arising from the cavity-mediated interaction.

Strictly speaking, the renormalised quasi-particle spectrum $\ep^{s}_{\bf k}$ in Eq.~(\ref{cavity-shifted-dispersion}) should be decided self-consistently via
\begin{equation*}
    \ep^{s}_{\bf k} = \ep_{{\bf k},1}^{d,U}  + \sum\limits_{s'} \int_{\bf k'} f^{s,s'}_{{\bf k},{\bf k'}}  n_F( \ep^{s}_{\bf k} - \mu )
\end{equation*}
where the Fermi function on the right hand side is given self-consistently. This self-consistency is necessary when the Landau interaction function $f^{s,s'}_{{\bf k},{\bf k'}}$ takes solely d-wave structure (see e.g. the discussion on $Sr_3 Ru_2 O_7$ in Ref.~\cite{rodriguez2013fermi}). This self-consistent treatment in our cavity-mediated interaction is no longer necessary, because here the dominating structure in $f^{s,s'}_{{\bf k},{\bf k'}}$ is the uniform s-wave, and the Fermi surface is extremely close to the bandtop (e.g., $k_F=\pi/30$). Under these conditions, by approximating the Fermi distribution $n_F( \ep^{s}_{\bf k} - \mu )$ by 1, we eliminate the need for self-consistency. In fact, under 0 temperature the result in Eq.~(\ref{cavity-shifted-dispersion}) is exactly the self-consistent result (because $\ep_{{\bf k'},1}^{d,U}$ and $\ep^{s}_{\bf k}$ gives the same Fermi surface), and we have not found any other self-consistent solution of $\ep^{s}_{\bf k}$ than the one in Eq.~(\ref{cavity-shifted-dispersion}).

For later use, we calculate the slope of $\ep^{s}_{\bf k}$ at the Fermi surface,
\begin{equation}\label{slope-at-FS}
\begin{split}
    \vert \nabla_{\bf k} \ep^{s}_{\bf k} \vert_{ {\bf k} \in FS } &= 
    (1+\eta) ~ \vert \nabla_{\bf k} \ep_{{\bf k},1}^{d,U} \vert_{ {\bf k} \in FS } 
    - \eta ~ \vert \nabla_{\bf k} \ep_{{\bf k},1} \vert_{ {\bf k} \in FS } \\
    &\approx (1+\eta)~ 2 \Tilde{t_1} k_F ~ - ~ \eta~ 2 t_1 k_F  
\end{split}
\end{equation}
where in the first line we insert the result of Eq.~(\ref{cavity-shifted-dispersion}), and in the second line we use the fact that $k_F=\pi/30$ is tiny, so that the dispersion relation $\ep_{{\bf k},1}$ near $k_F$ can be approximated by $ \ep_{{\bf k},1}\approx \ep_1 + 4 t_1 - t_1 \vert {\bf k}\vert^2 $, which is consistent with Eq.~(\ref{dispersion}). Similarly, near the tiny Fermi surface surrounding the $\Gamma$ point, we have $ \ep_{{\bf k},1}^{d,U}\approx \ep_{{\bf \Gamma},1}^{d,U} - \Tilde{t_1} \vert {\bf k}\vert^2 $, where we define $\Tilde{t_1} \equiv \Tilde{v_F} / (2 k_F)$ as the renormalised hopping parameter, and $\Tilde{v_F} =  \big\vert \nabla_{\bf q} \ep_{{\bf q},1}^{d,U} \big\vert_{\vert {\bf q}\vert = k_F} $ is the renormalised Fermi velocity.

Now, Eq.(\ref{deltaOmega}) and (\ref{Landau}) respectively matches the Eq.(2.1) and (3.20) in Ref.~\cite{rodriguez2013fermi}, we can thus directly use the criteria for the Pomeranchuk instability in Eq.(3.7) therein, which reads
\begin{equation}\label{criteria-in-ref}
    1 - \frac{1}{2\pi^2} \frac{\vert g   g_{c,{\bf q}={\bf 0}} \vert^2 }{ \Delta_c} \lambda^2 ~ \langle d \vert d\rangle ~ < ~ 0,
\end{equation}
where
\begin{equation}
    \lambda = \bigg( \frac{1}{4\pi^2} \int_{ \bf k } \frac{1}{ ( \Delta_{{\bf k},s} )^2 }  \bigg)^{1/2}
\end{equation} 
is the coefficient (in unit of unit $(\text{eV})^{-1}$) satisfying $\frac{1}{ \Delta_{{\bf k},s}  } = \lambda ~ d({\bf k})$, where $d({\bf k})$ is a basis function with same extended s-wave shape as $\frac{1}{ \Delta_{{\bf k},s}  }$, but satisfies the normalisation relation $ \frac{1}{4\pi^2} \int_{ \bf k } \big( d({\bf k}) \big)^2 =1  $. 
Here, according to Eq.~(3.1) in Ref.~\cite{rodriguez2013fermi}, we have
\begin{equation}\label{d-d-inner}
\begin{split}
    \langle d \vert d\rangle &\equiv \sum\limits_{s} \int_{\bf k} \delta \big(\mu-\ep^{s}_{\bf k} \big) ~ \big( d({\bf k}) \big)^2 \\
    &= \sum\limits_{s} \int_{ {\bf k}(l) \in FS}  dl  ~ \frac{ \vert \frac{d}{dl} {\bf k}(l) \vert }{\vert \nabla_{\bf k} \ep^{s}_{\bf k} \vert_{ {\bf k} = {\bf k}(l) } } ~ \big( d({\bf k}(l)) \big)^2 \\
    &\approx \sum\limits_{s} 2 \pi k_F \frac{1}{ (1+\eta)~ 2 \Tilde{t_1} k_F ~ - ~ \eta~ 2 t_1 k_F  } \big( d(\Gamma) \big)^2 \\
    &= 2 \pi \frac{1}{ (1+\eta)~  \Tilde{t_1}  ~ - ~ \eta~  t_1 } \big( \frac{1}{\lambda} \frac{1}{\Delta_{{\bf \Gamma},s}^{U}} \big)^2
\end{split}
\end{equation}
Here in the second line we parameterize the tiny Fermi surface by a line $l$ so that the above delta-function integral becomes a line integral on the Fermi surface (also see Ref.~\cite{rodriguez2013fermi}). In the third line use the fact that the tiny Fermi surface is can be well approximated by a circle with radius $k_F=\pi/30$, as well as the result in Eq.~(\ref{slope-at-FS}). We also approximate the basis function $d({\bf k}(l))$ by its value at the $\Gamma$ point which is also very accurate. In the last line we use the relation $\frac{1}{ \Delta_{{\bf k},s}  } = \lambda ~ d({\bf k})$. Inserting Eq.~(\ref{d-d-inner}) into Eq.~(\ref{criteria-in-ref}), we derive the criteria for the Pomeranchuk instability to appear in our cavity-material system:

\begin{equation}\label{appendix:Eq_Pomeranchuk-criteria}
    \frac{1}{\pi} \frac{\vert g   g_{c,{\bf q}={\bf 0}} \vert^2 }{ \Delta_c ( \Delta_{{\bf \Gamma},s}^{U} )^2 } >  \Tilde{t_1} ~ - ~ \eta ~ (t_1-\Tilde{t_1}) .
\end{equation}









\subsection{The excitonically enhanced cavity-mediated interaction favours the Pomeranchuk Instability}
To perform the Pomeranchuk analysis, we first focus on the mean-field effect (i.e. the electron-mass renormalisation) given by the cavity-mediated interaction (see Appendix \ref{appendix:Pomeranchuk-criteria}). We find the single particle spectrum is strongly renormalised by the forward scattering part of the excitonically screened cavity-mediated interaction, such that the van Hove singularity and the band-inversion is triggered much before the no-cavity ($g_c =0$) case. The excitonic screening strengthens this mean-field effect of the cavity-mediated interaction so strongly, that the van Hove point eventually appears earlier than the non-interacting case. In other words, the band-inversion is no longer postponed, when the contribution from the Floquet band-structure engineering and the cavity-mediated interaction is summed over.
%no longer need to \cite{lamas2008fermi,rodriguez2013fermi}

Following Ref.~\cite{rodriguez2013fermi}, in Appendix \ref{appendix:Pomeranchuk-criteria} we find (at zero temperature with near full occupation) %the exact condition for 
the cavity-mediated Pomeranchuk instability is triggered when
\begin{equation}\label{Pomeranchuk-criteria}
\frac{1}{\pi} \frac{\vert g   g_{c,{\bf q}={\bf 0}} \vert^2 }{ \Delta_c ( \Delta_{{\bf \Gamma},s}^{U} )^2 } >  \Tilde{t_1} ~ - ~ \eta ~ (t_1-\Tilde{t_1}).
\end{equation}
Here $\Tilde{t_1} \equiv \Tilde{v_F} / (2 k_F)$ is defined as the Floquet renormalised hopping parameter, where $\Tilde{v_F} =  \big\vert \nabla_{\bf q} \ep_{{\bf q},1}^{d,U} \big\vert_{\vert {\bf q}\vert = k_F} $ is the Floquet renormalised Fermi velocity and $k_F$ is the Fermi momentum. 
In our dipole coupling model, without cavity, $\Tilde{t_1}$ is suppressed as the driving strength $g $ approaches $\Delta_{\text{ex}}$. The van Hove singularity is created when this renormalised hopping vanishes, i.e., $\Tilde{t_1}\to0$. 
%Meanwhile 
%It can be further suppressed by other dynamical localisation mechanisms which are not considered in our present model. 
In the presence of the cavity-mediated interaction, the single-particle spectrum (deciding the electron's thermal occupation) is further flattened (see Eq.~\ref{cavity-shifted-dispersion}), and the overall effective hopping parameter near the Fermi surface becomes the right hand side of Eq.~(\ref{Pomeranchuk-criteria}).
In Eq.~(\ref{Pomeranchuk-criteria}) there is an important factor $\eta$, defined in Eq.~ (\ref{appendix:eta-param}) as
\begin{equation}\label{main:eta-param}
\begin{split}
\eta &\approx \frac{1}{\pi^2} \frac{\vert  g_{c,{\bf q}={\bf 0}} \vert^2 }{ \Delta_c} \int_{\bf k'} \frac{1}{ \Delta_{{\bf k'},s'} }.
\end{split}
\end{equation}
This factor is the product of the cavity-coupling parameters with the s-wave strength of $\frac{1}{ \Delta_{{\bf k},s}}$. When the driven material is coupled to the cavity, the cavity-mediated interaction further contributes a self-energy (mean-field correction) to the single-electron energy $\ep_{{\bf q},1}^{d,U}$ defined in Eq.~(\ref{eq.h_eff}). This cavity correction is given by $- \eta \frac{\vert g \vert^2}{\Delta_{{\bf q},s}} $, i.e., it effectively enhances the optical Stark shift by a factor of $\eta$. Physically, the momentum integration in $\eta$ in Eq.~(\ref{main:eta-param}) means that, an electron's energy is decreased by electrons at all other momenta $\bf k'$ via the cavity-mediated interaction. We can already estimate from Fig.~\ref{fig.interaction} that, in the interacting case, this $\eta$-factor will be stronger than the non-interacting case by an order of magnitude. This great enhancement can again be explained by the momentum-mixture mechanism: via the formation of virtual excitons in the cavity-mediated interaction, electrons with momenta far from the Fermi surface are now effectively contributing to the Fermi-surface deformation. 

In Fig.~\ref{fig:Pomeranchuk} we fix the driving strength $g =0.05$eV, and plot the two sides of Eq.~(\ref{Pomeranchuk-criteria}) as a function of the laser detuning to the resonance. For the interacting model (blue curves) this is the laser-exciton detuning $\Delta_{\text{ex}}$, and for the non-interacting case this is the laser-bandtop detuning $\Delta_{\text{gap}}$. Here the thick curve represents the left part of Eq.~(\ref{Pomeranchuk-criteria}) proportional to the interaction strength at $\Gamma$ point, the dot-dashed curve represents the right part of Eq.~(\ref{Pomeranchuk-criteria}), and the dashed curve represents the Floquet renormalised hopping parameter $\Tilde{t_1}$ without cavity contribution. The Pomeranchuk instability is triggered as the thick curve crosses the dot-dashed curve, before the van Hove singularity is created as the dot-dashed curve becomes negative. 
Compared with the non-interacting case (blue versus red), we identify the three above-mentioned excitonic screening effects: the postpone of van Hove singularity by the driving without the cavity (i.e. the dashed line is moved rightward), the strong enhancement on the factor $\eta$ describing the self-energy correction from the screened cavity-mediated interaction (i.e. the displacement from the dashed to the dot-dashed line is strongly enlarged), and the enhanced interaction strength at $\Gamma$ point (i.e. the thick line is moved upward). 
According to Fig.~\ref{fig:Pomeranchuk}, (in the interacting case with $k_F=\pi/30$ and $g =0.05$eV) we estimate this instability is triggered for a laser-exciton detuning at $\Delta_{\text{ex}}=0.14$eV (close to the van Hove singularity, where the right side of Eq.~(\ref{Pomeranchuk-criteria}) becomes negative), where the laser-cavity detuning is $\Delta_c=0.25$eV with electron-cavity coupling $ g_{c,{\bf q}={\bf 0}} = \sqrt{N} g_{c,{\bf R}} =0.1$eV. 
According to Refs.~\cite{lamas2011pomeranchuk,rodriguez2013fermi}, we estimate that under these parameters, this instability can still be triggered as the temperature increases to $k_B T\sim \big( \Tilde{t_1} - \eta(t_1 -\Tilde{t_1}) \big) (k_F)^2\sim 1$ Kelvin. 
Here $\big( \Tilde{t_1} - \eta(t_1 -\Tilde{t_1}) \big) (k_F)^2$ represents the Fermi energy for holes, which becomes 0 as the van Hove singularity is created cooperatively by driving and cavity-mediated interaction. 

If we instead simulate a non-interacting electron system (red curves in Fig.~\ref{fig:Pomeranchuk}) with the same driving strength, we would have to push the driving frequency even closer to the van Hove singularity, in order to compensate for the weaker cavity-mediated interactions. 
%this makes $\Tilde{t_1}$ small enough so that the weak unscreened cavity-mediated interaction can also trigger the Pomeranchuk instability. 
Furthermore, in this non-interacting case, as $\Tilde{t_1}$ becomes much smaller, the instability only survives below a lower temperature $k_B T\sim \big( \Tilde{t_1} - \eta(t_1 -\Tilde{t_1}) \big) (k_F)^2 \sim 0.2$ Kelvin. 
This comparison shows that, the excitonic screening enhances the cavity-mediated s-wave Pomeranchuk instabilities in two aspects: First, the overall shift of the van Hove singularity makes the instability easier to trigger (at a larger detuning), and, second, the enhanced interaction strength at the $\Gamma$ point allows the triggered instability to survive at larger temperatures.

In the interacting case, by choosing a smaller driving strength ($g =0.02$eV in Fig.~\ref{fig:Pomeranchuk-weak} and $g =0.01$eV in Fig.~\ref{fig:Pomeranchuk-weakest}), the instability can be triggered at slightly higher temperature, as we tune the driving frequency closer to the exciton resonance. For $g =0.02$ eV we find the instability is triggered at $\Delta_{\text{ex}}\approx0.056$ eV, and for $g =0.01$ eV it is triggered at $\Delta_{\text{ex}}\approx0.029$ eV. However, in this near resonance strong driving case, higher-order correction in $g $ (i.e. the virtual bi-exciton effect) should be considered in the effective Hamiltonian as well. Besides, in reality, the exciton line-width in the absorption spectrum sets up a lower limit of $\Delta_{\text{ex}}$.
%requires further examination which includes higher-order ($\vert g \vert^4$) virtual exciton-related driving effects. 
As a comparison, in the non-interacting case, we see that the temperature at which the instability can be observed remains to be much lower than the interacting case, no matter how small the driving strength we choose. 

The electron-cavity coupling $g_c\lesssim0.05$ eV we used here is achievable due to the large electric dipole in the organic molecules, see e.g  Ref.~\cite{frisk2019ultrastrong} for a list of cavity-molecule setups where vacuum Rabi splitting of $\sim1$ eV is realised. Moreover, if the electrons are coupled to several cavity modes with similar detuning $\Delta_c$, the forward scattering will increase with the mode numbers, this will make the instability happen at much larger laser-exciton detuning.

In deriving the criteria for the Pomeranchuk instability in Eq.~(\ref{Pomeranchuk-criteria}), we have omitted the contribution given by the Hubbard term $\hat{U}_{11}$. First, at such a low carrier density, its contribution to the single-particle dispersion is, apart from a chemical potential shift, is a slight electron-mass renormalisation $\Tilde{t}\to \Tilde{t} / (1+ 2 (-\ln{n_h})^{-2}) $ which can hardly be observed in the above figures. 
In addition, after the ladder series renormalisation\cite{arovas2022hubbard,engelbrecht1992landau} which is exact in the dilute limit, the Hubbard term could only contribute an effective repulsion $U_{\text{eff}} \sim \Tilde{t_1} (-\ln{n_h})^{-1}$, which is much smaller than its bare value $U_{11}$. This effective repulsion $U_{\text{eff}}$ cannot compete with the cavity-mediated attractive interaction under the parameters considered above, i.e. $U_{\text{eff}}$ is smaller than the cavity-mediated interaction roughly by an order of magnitude. Thus the above result is almost quantitatively unchanged after including the on-site repulsion $\hat{U}_{11}$ term in Eq.~(\ref{eq.U_eff}) into the Pomeranchuk analysis.

%No longer useful as this is close to half-filling: On the RPA level (see Ref.~\cite{frigeri2002landau}), the repulsive Hubbard term $\hat{U}_{11}$ can give attractive contribution to the forward-scattering channel for large enough $U_{11}$, which might furthermore facilitate the Pomeranchuk instability predicted above. 

In experiments with weaker driving strength, larger laser-exciton detuning and higher temperatures, this excitonically-enhanced cavity-mediated interaction itself may only be able to soften the Fermi-surface instead of deforming it. But this interaction should already show a strong influence on the dynamical responses, like Boltzmann transport and the zero sound~\cite{chan2010anisotropic}, before the Pomeranchuk instability appears. 
%{\Large $\lambda^i$}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{images/exciton-revisited/Pomeranchuk.png} \captionsetup{justification=raggedright,singlelinecheck=false}
    \caption{ Pomeranchuk instability, $g =0.05$ eV. The thick line represents the cavity-mediated interaction, Pomeranchuk instability appears as it becomes larger than the dot-dashed line, which represents the overall effective hopping parameter. The bare Floquet (no-cavity) contribution of this effective hopping parameter, $\Tilde{t_1}$, is represented by the dashed curve. 
    The blue curves represent the 3 above-mentioned quantities in the interacting model with horizontal axis representing the laser-exciton detuning $\Delta_{\text{ex}}$, the red curves represent these 3 quantities in the non-interacting model with horizontal axis representing the laser-bandtop detuning $\Delta_{\text{gap}}$. 
    Both axes are in the unit of eV.
    }
    \label{fig:Pomeranchuk}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{images/exciton-revisited/Pomeranchuk-weak.png} \captionsetup{justification=raggedright,singlelinecheck=false}
    \caption{ Pomeranchuk instability, $g =0.02$ eV }
    \label{fig:Pomeranchuk-weak}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{images/exciton-revisited/Pomeranchuk-weakest.png} \captionsetup{justification=raggedright,singlelinecheck=false}
    \caption{ Pomeranchuk instability, $g =0.01$ eV }
    \label{fig:Pomeranchuk-weakest}
\end{figure}


